How to Optimize the Environmental Impact of Transformed NoSQL Schemas through a Multidimensional Cost Model?

The complexity of database systems has increased significantly along with the continuous growth of data, resulting in NoSQL systems and forcing Information Systems (IS) architects to constantly adapt their data models (i.e., the data structure of information stored in the database) and carefully choose the best option(s) for storing and managing data. In this context, we propose %in this paper an automatic global approach for leading data models' transformation process. This approach starts with the generation of all possible solutions. It then relies on a cost model that helps to compare these generated data models in a logical level to finally choose the best one for the given use case. This cost model integrates both data model and queries cost. It also takes into consideration the environmental impact of a data model as well as its financial and its time costs. This work presents for the first time a multidimensional cost model encompassing time, environmental and financial constraints, which compares data models leading to the choice of the optimal one for a given use case. In addition, a simulation for data model's transformation and cost computation has been developed based on our approach.

==> BDA2020_Demo/files/01-Introduction.tex <==
\section{Introduction}
\label{Introduction}

For many decades, the storage and the exploitation of data has mainly relied on relational databases. With the advent of Big Data, the volume of data has exploded, the heterogeneity has increased tenfold, causing problems of transformation from traditional data\-bases to new storage on the Cloud, whether in terms of storage management, data query, cost or performance. To deal with these problems, new data management systems called \emph{NoSQL} systems have appeared since 2009.

The phenomenon of data explosion, characterized by the \texttt{5V} (Volume, Variety, Velocity, Veracity, and Value), has opened up major research themes based on modeling, manipulation and storage of massive amounts of data~\cite{tauro2012}.
Storage methods have led to the definition of specific data models, corresponding to four families of data structures: key-value oriented (\texttt{KVO}), column oriented (\texttt{CO}), document oriented (\texttt{DO}) and graph oriented (\texttt{GO}). %The choice of the most suitable NoSQL family and of its implementation is a crucial task.  

Several works have focused on storage and modeling problems of data using NoSQL systems. Most of the studies have proposed either (i) a comparative study between RDB (Relational DataBases) and NoSQL DB (DataBases) and/or how to transform relational data into dedicated NoSQL system \cite{li2010,vajk2013,rocha2015} or (ii) how to transform a conceptual schema into a specific NoSQL DB \cite{abdelhedi2017,Gwendal2019,daniel2016umltographdb,li2014,hamouda2017,claudino2016} (iii) while very few studies have proposed criteria for the choice of physical models and implementation platforms \cite{jatana2012,tauro2012,raut2017}.

Our \DG~\cite{EGC20_dataguide,DEXA20_dataguide} approach offers logical modeling suitable for models refinement in order to generate all types of optimized physical models by relying on a common \MMFF~meta-model (4 NoSQL families \& the Relational model). Based on transformation rules, it provides a functional process that integrates the use case to generate the different SQL and/or NoSQL solution(s) adapted to business requirements. %The contributions of this work are:
%\begin{itemize}
  %\item An approach that subtly combines conception with optimization in databases transformation process,
  %\item A common meta-model dedicated to support all families (relational and NoSQL) and schema transformation,
 %\item A heuristic to reduce the search space of data model generation.
%\end{itemize}

\DG~favors the flexibility of the schema offered by NoSQL DB as a whole and allows going from one model to another, or from one family to another \textit{via} refinements; merging several source concepts into a single target concept, or splitting a source concept into several target concepts. Thus, the meta-model's flexibility has been sufficiently exploited to facilitate transformations and improve performances.

This paper develops our \DG~approach, the \MMFF{} meta-model and refinement rules in Section~\ref{sec:approach}. We demonstrate the use of refinement rules and possibilities offered by our common meta-model in Section~\ref{sec:Demonstration}. Finally, a conclusion opens the research perspectives in Section~\ref{sec:conclusion}.



==> BDA2020_Demo/files/02-Approach.tex <==
%\externaldocument[contribution]{05_contribution}
\section{\DG: From Conceptual Model to Physical Models}
\label{sec:approach}

\begin{figure*} [t]
    \includegraphics[width=.845\linewidth]{BDA2020_Demo/images/DataGuide_Process.pdf}
	\caption{\DG~Approach\label{fig:process}}
\end{figure*}

We suggest a model driven approach that offers steps to generate a logical model for each family. %(the relational \& 4 NoSQL). 
Our approach focuses on model transformation, starting from conceptual to logical then to physical models, and on model refinement to go from one logical model to another. 
The peculiarity of this approach is to allow the optimization of the data model directly during the transformation process instead of the last step. This helps to make a choice of implementation according to the context of use. 
In order to formalize the implementation of models, we adopted a Model-Driven Architecture (MDA\footnote{https://www.omg.org/mda/index.htm}) that offers 3 types of models, namely 1) the \textit{Computation Independent Model} (\texttt{CIM}) which allows to describe the requirements, 2) the \textit{Platform Independent Model} (\texttt{PIM}) that describes the components of the system independently of platforms, 3) and the \textit{Platform Specific Model} (\texttt{PSM}) which describes the components of the system using a precise technical platform.
MDA also recommends transforming models using the formalization of transformation (or refinement) rules in language such as \textit{Query-View-Transformation} (\texttt{QVT})\footnote{https://www.omg.org/spec/QVT/About-QVT/}. 

In our \DG~approach (depicted in Figure~\ref{fig:process}), as we start from a UML class diagram, we consider two Platform Independent levels corresponding to the conceptual (PIM1) and logical (PIM2) levels, as well as a Platform Specific level related to the different target platforms. We mention that, the input of our approach is the UML class diagram which is usually considered as a PIM that could be automatically transformed into a target PSM, substituting the CIM less adapted in this work. 
%Our illustrated in Figure~\ref{fig:process} and defined as follows:
 
 %In our \DG~approach, we provide  consists of two PIM levels and a PSM level, illustrated in Figure~\ref{fig:process} and defined as follows:
 
The \textbf{PIM1} (\textit{Platform Independent Model}) of the first level integrates the functional needs of the IS, both in terms of data and queries. This UML class diagram serves as a basis for modeling the user requirements and the context of use. 
%We needed this class diagram's meta-model to be as platform independent as possible, in order to be suitable with a number of different platforms. %not only the one we are describing.
%\remJ{CIM vs PIM1}

 
The \textbf{PIM2} is the second level independent model, common to the five families of models.
It allows to carry out \textit{refinement} rules by generating recursively all possible denormalized models by relying on merge and split rules.
We mention that a heuristic is applied to guide the generation of data models in order to avoid cycles and useless models.
It is mainly based on the use case.
This heuristic is not detailed in this demonstration.
 
The \textbf{PSMx} (\textit{Platform Specific Model}) are obtained by the transformation of PIM2 models into the compatible target data family (e.g. nesting for \texttt{DO}, rows for \texttt{CO}, edges for \texttt{GO}, etc.). 
 %not clear ...!

This demonstration focuses especially on the \texttt{PIM2} \MMFF{} meta-model used to generate all possible data models, on transformation, and on refinement rules.


%The latter is the standard proposed by the OMG for models transformation.

%\remNT{Comme dit par un rapporteur, bien mettre en valeur la différence entre CIM et PIM1}


==> BDA2020_Demo/files/03-Common_metamodel.tex <==
\subsection{A Meta-Model to Unify the 5 Families}

 \begin{figure*}[t]
	\includegraphics[width=.84\linewidth]{BDA2020_Demo/images/MM5F.jpg}
	%\caption{PIM2 \MMFF{} Meta-Model Common for the 5 families of data models\label{fig:PIM2}}
	\caption{PIM2 Common \MMFF{} Meta-Model (Relational \& NoSQL 4 Families)  \label{fig:PIM2}}
\end{figure*}

The common meta-model (PIM2 level) is the cornerstone of our approach. This meta-model provides a common representation of all the concepts of the five families, and allows all the possible \textit{refinements} within the same family or between two different families. 
%integrates all possibilities of data schema \textit{refinement}. 
In this section, we introduce the PIM2 meta-model, and we present some of the \textit{refinement} rules.

\subsubsection{\MMFF{} Meta-Model. }
\label{sec:metamodel}

The common meta-model seeks to produce different models compatible with the PSM constraints while remaining independent. The subtlety of the PIM2 meta model is to integrate all the different concepts of the five families.
A major advantage of this meta-model is that, if a denormalization (or normalization) solution proves to be well suited to a case of study using a given family, this solution can possibly be adapted to the four other families.
Based on \textit{refinement} rules, merges or splits of concepts will be applied in order to adapt them to a relational, key-value, column, document or graph oriented data models.

Figure~\ref{fig:PIM2} shows the proposed PIM2 \MMFF{} meta-model which embeds the different concepts used in the 5 families data models: concepts contain rows (for column-oriented models), key-values with simple or complex values, and edges to facilitate the integration of graph databases.

Complex Values are represented by the composition of rows. A loop occurs between rows and complex values in the meta-model, it shows that a value can be multiple and its schema is structurally identical to a concept. The key point of this modeling, is to enable the application of refinement rules without iteration limits, allowing the production of schemas which helps to find most suitable ones according to a given use case. Meta-constraints are associated to the Complex Value to prevent the mutual composition of instances.

%Constraints and references are associated with keys, which can belong to distinct concepts. The idea is to be able to transform these constraints into new representations using refinement rules. For example, a \textit{Reference} can be transformed into an \textit{Edge} for graph-oriented models or into a \textit{Foreign Key} in relational databases.
\begin{figure}[t]
%\begin{minipage}{.8\linewidth}
	\centering\includegraphics[width=1\linewidth]{BDA2020_Demo/images/RowsConceptToRowConcept.pdf}
	\caption{Concepts' Rows merge QVT rule \label{fig:merge}}
%\end{minipage}
\end{figure}

\subsubsection{Common Model Transformation and Refinement. }
\label{sec:transformations}

Thanks to the common meta-model, refinement can be applied iteratively while respecting the meta-model. PIM2 refinement relies on three transformation rules:
\begin{itemize}
  \item \textbf{Merge} \textit{rows} between concepts to produce \textit{complex values} for nesting (\texttt{CO}, \texttt{DO}) or to merge keys for values %concatenation 
  (\texttt{KVO}),
  \item \textbf{Split} \textit{rows} to produce new columns in a same \textit{concept} (\texttt{CO}),
  \item \textbf{Transform} \textit{references} into the equivalent \textit{edges} (\texttt{GO}).
\end{itemize}

Figure~\ref{fig:merge} shows the \texttt{Row\-Concepts\-To\-Nested\-Row\-Concept} rule, a refinement QVT rule that merges rows belonging to two different concepts. Thus, two rows from two different concepts referring to each other (initially classes associated at the PIM1 level) can be merged into a single row with a complex value. 
Row \textit{r2} of concept \textit{co2} is linked by reference \textit{ref} to concept \textit{co1} through row \textit{r1}. To merge rows, row \textit{r2} is then nested into a complex value \textit{cv} which corresponds to the transformation of the reference into a new key value \textit{k}. The latter corresponds to the transformation of the reference key \textit{k1}.
%This rule can be applied in both directions by switching \textit{co1} and \textit{co2} (generating a list of complex values in~\textit{k}).

%Figure~\ref{fig:split} illustrates the \texttt{RowConceptTo\-RowsConcept} split refinement rule. It shows that a key value \textit{k} linked to a row \textit{r} can be separated from it and placed in a new row \textit{r2} which is linked to the same concept. This split represents the fact that several rows can occur for a same concept (\textit{i.e.,} a column family in \texttt{CO}). We notice that the primary key constraint \textit{c} is duplicated in the new row \textit{r2} to preserve uniqueness and to allow instances reconstructions when instances will be physically separated.
%The content of row \textit{r} remains unmodified except for the moved key value \textit{k}, which means that remaining key values from \textit{r} are still linked to \textit{r} (called \textit{r1} in the target data model).
%The rule \texttt{RowConceptToRowsConcept} can also be applied on a set of key values to move this set into \textit{r2}.

%As detailed in the following, the generation of data models will rely on those rules by applying them recursively on various combinations of transformations.
%However, the number of possibilities is infinite, because each succession of refinement operation can find its opposite to reproduce the original diagram, and thus generate a cycle.
%Each new schema produced by QVT rules can be transformed to target PSMx.




==> BDA2020_Demo/files/04-1-Experimental_Environment.tex <==
\subsubsection{Experimental Environment. }

Since our approach is based on (MDA\footnote{MDA: \url{https://www.omg.org/mda/index.htm}}), we need an infrastructure suitable for meta-modeling, modeling and models transformations. We developed our approach using a model transformation environment called \textit{Eclipse Modeling Framework} (EMF\footnote{EMF: \url{https://www.eclipse.org/modeling/emf/}}). It is a set of Eclipse plug-ins which can be used to design a data model and to generate code or other output based on this model. EMF respects the known distinction between a meta-model and a model. 
A meta-model describes the structure of a model. A model is a concrete instance of this meta-model. To implement our approach, we have used  the following tools proposed by EMF: 1) \textit{Ecore} used for the implementation of all the \texttt{PIM1}, \texttt{PIM2}, and \texttt{PSMx} meta-models. Inspired by the object-oriented approach, the Ecore language is based on the notion of package (EPackage), class (EClass), attribute (EAttribute), reference link (EReference), data type (EDataType), and enumeration (EEnum); 2) \textit{XMI}\footnote{\textit{XML Metadata Interchange}: \url{https://www.omg.org/spec/XMI/About-XMI/}} a format in which instances of meta-models are created; and 3) \textit{QVTO} (QVT Operational) a Model-To-Model (M2M) transformation tool that implements the QVT language.
%\textit{QVT} a Model-To-Model (M2M) transformation language proposed by OMG. 
It is used to formalize both exogenous transformation rules (from conceptual to logical model, and from logical to physical model) and also refinement (endogenous transformation) rules.

==> BDA2020_Demo/files/04-Implementation.tex <==
\subsection{Implementation}

%In order to illustrate our approach, we used the TPC-C\footnote{TPC-C: \url{http://www.tpc.org/TPC-C/default.asp}} benchmark giving a full use case mixing at the same time transactions, joins and aggregations.
%The TPC-C benchmark simulates the behavior of a logistic DB on user orders with transaction-oriented stock management (OLTP). We will focus on the six classes (\textit{Warehouse}, \textit{District}, \textit{Customer}, \textit{Order} and \textit{OrderLine}, \textit{Item}) as illustrated in the PIM1 depicted in Figure~\ref{fig:PIM1}.

%In order to illustrate our approach, we generated different denormalized schemas that we have integrated into a \texttt{MongoDB} database.
%The choice was led by the fact that \texttt{MongoDB} is one of the rare NoSQL solutions integrating ACID transactions in \textit{sharding} (version 4.2) required by the TPC-C benchmark.
%However, our approach is extensible by defining a new PSM for each target database type (without ACID properties in that case).

The implementation of our approach presented in this demonstration enlightens the models generation process by showing the three main interactions: 1) \textit{Conceptual Model} to \textit{Common Logical Model} Transformation; 2) \textit{Common Logical Model Refinement}; 3) \textit{Common Logical Model} to \textit{Physical Model} Transformation.
The whole process shows how applying the \DG{} approach generates different data models based on the entry class diagram expressing the use case using transformation/refinement rules.

%The transformation process is illustrated by the TPC-C\footnote{TPC-C: \url{http://www.tpc.org/TPCC/default5.asp}} benchmark.
%It gives a full use case mixing at the same time transactions, joins and aggregations.
%The TPC-C benchmark simulates the behavior of a logistic DB on user orders with transaction-oriented stock management (OLTP). We will focus on the six classes (\textit{Warehouse}, \textit{District}, \textit{Customer}, \textit{Order} and \textit{OrderLine}, \textit{Item}) as illustrated in the PIM1 depicted in Figure~\ref{fig:PIM1}.

\begin{figure} [t]
    \includegraphics[width=1\linewidth]{BDA2020_Demo/images/Ecore.pdf}
	\caption{Conceptual, Logical and Physical Ecore Meta-Models
	\label{fig:ecore}}
\end{figure}

\subsubsection{ConceptualMMtoLogicalMM Transformation}
\label{subsec:cmm2lmm}

In this section, we present the \texttt{ConceptualMM\-to\-LogicalMM} Transformation, which is the first step of our approach shown in Figure~\ref{fig:process}. 

\textbf{Source.} The source is the conceptual meta-model (PIM1) which, in our case, is a simplified UML\footnote{UML: \url{https://www.omg.org/spec/UML/2.5.1/PDF}} class diagram meta-model shown in (a) of Figure~\ref{fig:ecore} implemented in Ecore\footnote{\textit{Ecore}: \url{https://www.eclipse.org/ecoretools/overview.html}}.


\textbf{Target. } The target is the \MMFF{} Meta-Model used for model transformation and proposed in Section~\ref{sec:approach}.
Our meta-model is formalized in \textit{Ecore} as shown in (b) of Figure~\ref{fig:ecore} in order to verify all transformations and refinements of models.
%\remNT{destination : Une instance du MM}
%\remNT{Adaptations particulières ?}

\textbf{ConceptualMMtoLogicalMM Transformation. } UML classes, associations, etc. from the PIM1 (Conceptual Meta-Model) are transformed into concepts, references, etc. of our PIM2 (\MMFF{} Meta-Model) respectively. Rules are expressed in \texttt{QVT} language.

%This step is illustrated by the transformation of the class diagram model represented in Figure~\ref{fig:conceptual_m} into the output model defined in Figure~\ref{fig:logical_m} corresponding to the \MMFF~meta-model.
%\remNT{illustrations avec TPC-C pour la démo ? Garder les MM pour l'implémentation et les modèles pour illustrer la démo.}


\begin{figure}[t]
	\includegraphics[width=1\linewidth]{BDA2020_Demo/images/PIM1_TPCC.png}
	\caption{PIM1 of TPC-C Benchmark\label{fig:PIM1}}
\end{figure}

\subsubsection{\MMFF{} Meta-Model Refinement}
\label{subsec:Refinement}

At PIM2 level, models' refinement uses endogenous transformations where both source model and target model are instances of the same meta-model, here the \MMFF{} meta-model.

\textbf{Source.} The source meta-model for this transformation is the \MMFF{} meta-model. %(Ecore implementation in Figure~\ref{fig:logical_mm}).

\textbf{Target.} Each refinement applied to the PIM2 meta-model produces an instance data model of the \MMFF{} meta-model (relational, key-value, column, document or graph oriented).

\textbf{\MMFF~Meta-Model Refinement.} Three rules can be applied to a \MMFF{} data model: Merge, Split and References to edge.
Each one is a refinement rule implemented in QVT in order to generate all denormalized data models.
The generation of data models by recursive applications of refinement rules is bounded by a heuristic detailed in~\cite{DEXA20_dataguide} and produces a tree of data models.

Figure~\ref{fig:merge} corresponds to the merge between two rows from different concepts referring to each other by transforming a reference into a nested key-value. We can also apply a split rule that will detach two keys from a given PIM2 data model into two rows linked to the same concept. 

The input of the transformation script for each refinement is a PIM2 instance. However, the heuristic begins with the output of the \texttt{ConceptualMMtoLogicalMM} Transformation (Section~\ref{subsec:cmm2lmm}).
%All output data models are implemented in the \texttt{XMI} format and are compatible with the \MMFF{} meta-model.

\subsubsection{LogicalMMtoPhysicalMM Transformation. }
\label{subsec:lmm2pmm}

After obtaining the different logical models from the \MMFF~common meta-model refinement, we transform them into suitable physical models related to the corresponding PSM meta-model. In our case, we transform our relevant data models into \texttt{MongoDB} model.
The \texttt{MongoDB} meta-model is implemented in Ecore as stated in (c) of Figure~\ref{fig:ecore}.
This exogenous transformation is the last step in our \DG~process.

\textbf{Source. } The source is one of the data models generated by the refinement script discussed in Section~\ref{subsec:Refinement}.

\textbf{Target. } For the given logical model, the target is going to be one of the PSM meta-models.

\textbf{LogicalMMtoPhysicalMM Transformation.} In order to achie\-ve this, a QVT rule is defined for each PSM meta-model.
For the PSM of \texttt{MongoDB}, we transform \texttt{Concepts} to \texttt{Collec\-tions}, \texttt{Rows} to \texttt{Documents},   \texttt{Complex Values} to \texttt{Nested documents}, etc. %(for more details, see~\cite{abdelhedi2017}).

\input{BDA2020_Demo/files/04-1-Experimental Environment}

%\subsubsection{Implementation of Transformations}

%The \DG{} approach is composed of all meta-models in Ecore (PIM1, PIM2, and MongoDB PSM) and also of QVT rules for transformations, and refinements.
%The process to implement a given data model relies on the following steps: 
%\begin{enumerate}
   % \item Create an instance of the source meta-model in the XMI format, in our case the source is the conceptual meta-model, and as an instance, we will use the TPC-C class diagram, shown in Figure~\ref{fig:PIM1}.
    %\item Typically, transform the PIM1 into the PIM2 as a  normalized relational model
    %\item Apply the heuristic to generate a tree of denormalized data models (using recursively refinement rules)
    %\item Choose one or more generated PIM2, and apply its transformation into the target PSM
%\end{enumerate}
%\remNT{J'ai réécrit pour séparer l'implémentation du processus (offline) et de l'application du processus (online).}

\begin{comment}
\begin{figure}[t]
\begin{minipage}[b]{.325\linewidth}
	\fcolorbox{black}{white}{
	%\includegraphics[width=.9\linewidth]{BDA2020_Demo/images/Ecore_UML_MM.pdf}}
	\includegraphics[width=.9\linewidth]{BDA2020_Demo/images/EcoreUMLMM.png}}
	\caption{Ecore Class Diagram Meta-Model \label{fig:conceptual_mm}}
\end{minipage}
\hfill
\begin{minipage}[b]{.325\linewidth}
    \fcolorbox{black}{white}{
    %\includegraphics[width=.9\linewidth]{BDA2020_Demo/images/Ecore_5F_MM.pdf}}
    \includegraphics[width=.9\linewidth]{BDA2020_Demo/images/EcoreCommonMM1.png}}
    \caption{Ecore Logical Meta-Model \label{fig:logical_mm}}
\end{minipage}
\hfill
\begin{minipage}[b]{.325\linewidth}
    \fcolorbox{black}{white}{
    %\includegraphics[width=.9\linewidth]{BDA2020_Demo/images/Ecore_MONGODB_MM.pdf}}
    \includegraphics[width=.9\linewidth]{BDA2020_Demo/images/EcoreMONGODBMM.png}}
    \caption{Ecore Physical Meta-Model \label{fig:physical_mm}}
\end{minipage}
\end{figure}
\end{comment}

==> BDA2020_Demo/files/05-Demonstration.tex <==

\section{Demonstration}
\label{sec:Demonstration}
\fboxsep=0mm
\fboxrule=1pt

Before starting the transformation process, it is necessary to define the three meta-models that we have in our \DG~ approach shown in Figure~\ref{fig:process} since they are going to be needed in any further steps. We defined the conceptual (class diagram), logical (\MMFF) and physical (MongoDB) meta-models using \texttt{Ecore} as illustrated in Figure~\ref{fig:ecore}.
We also formalized the transformation/refinement rules in QVT (Query/View/Trans\-formation).

\subsection{TPC-C Benchmark Scenario}

For this scenario, we have used the TPC-C\footnote{TPC-C: \url{http://www.tpc.org/TPCC/default5.asp}} benchmark as an entry.
It gives a full use case mixing at the same time transactions, joins and aggregations.
The TPC-C benchmark simulates the behavior of a logistic DB on user orders with transaction-oriented stock management (OLTP). We will focus on the six classes (\textit{Warehouse}, \textit{District}, \textit{Customer}, \textit{Order} and \textit{OrderLine}, \textit{Item}) as illustrated in the PIM1 depicted in Figure~\ref{fig:PIM1}.

We started this demonstration by instantiating the PIM1 meta-model %(\texttt{Conceptual meta-model}) of our \DG~process 
using TPC-C benchmark's class diagram represented in (a) of Figure~\ref{fig:xmi}. TPC-C gives a full use case that helps us to test our approach. The benchmark's class diagram served as the entry for the \texttt{ConceptualMM\-to\-LogicalMM} transformation. After applying this transformation, it resulted in a model suitable to our \MMFF~common meta-model that is shown in (b) of Figure~\ref{fig:xmi}.

The next step refines the resulted model. Starting by the logical model derived from the first transformation rule, and by applying different refinement rules, we can obtain various models compatible with the PIM2 \MMFF{}. During the demonstration, we applied semi-automatic refinement rules (see Section~\ref{subsec:Refinement}).

\begin{figure} [t]
    \includegraphics[width=1\linewidth]{BDA2020_Demo/images/XMI.pdf}
	\caption{Class Diagram, \MMFF{} \& MongoDB XMI Models \label{fig:xmi}}
\end{figure}

We finally transform the model obtained from the refinement into a \texttt{MongoDB} database as shown in (c) of Figure~\ref{fig:xmi}.
The choice was led by the fact that \texttt{MongoDB} is one of the rare NoSQL solutions integrating ACID transactions in \textit{sharding} (version 4.2) required by the TPC-C benchmark.
However, our approach is extensible by defining a new PSM for each target database type (without ACID properties in that case). We can also visualize the JSON schema of the final output.

\subsection{User Model Scenario}

This scenario illustrates the whole process by integrating user's own data model.
The user has to follow the undermentioned steps while using the \DG~Approach:
\begin{enumerate}
    \item Create its own instance of the source meta-model in the XMI format, in our case the source is the conceptual class diagram meta-model,
    \item Typically, transform the PIM1 into the PIM2 as a  normalized relational model,
    \item Apply the heuristic to generate a tree of denormalized data models (using recursively refinement rules),
    \item Choose one or more generated PIM2, and apply its transformation into the target PSM.
\end{enumerate}

First, the user needs to specify his needs. These needs are then formalized in a UML class diagram and entered as an instance of the PIM1 class diagram meta-model by the user. %that we created in our \DG~process. 
This instance is defined in XMI format. The user runs then the first transformation (\texttt{ConceptualMM\-to\-LogicalMM}) script. 
As a result he obtains is a relational model corresponding to the \texttt{5Fami\-lies} meta-model.

The user runs the refinement script afterwards. The input of this script is automatically the model resulted from the \texttt{ConceptualMM\-to \-LogicalMM} transformation. The use of refinement rules shows how we can generate plenty of models. However, the number of solutions can explode since splits can be applied on each key and merges can be done in several ways. Therefore, the heuristic reduces the search space that is going to be displayed to the user as a tree of possible solutions generated by the multiple refinement rules applied on the model. The user can then pick out of the solutions proposed to him the one that he prefers. %showing the chaining of the applied refinement rules. The user can then pick out of the different solutions proposed the one that he prefers.

Finally, the user runs the last transformation script ( \texttt{LogicalMM\-to\-PhysicalMM}). The input of this script is the output of the \textit{refi\-nement} script chosen by the user. At the end, the user obtains the final model which is a result of transforming the model that he chose, from the tree of solutions, into the suitable physical model. 


\begin{comment}
\begin{figure}[t]
\begin{minipage}[b]{.320\linewidth}
	\fcolorbox{black}{white}{\includegraphics[width=1\linewidth]{BDA2020_Demo/images/%instance_UML.pdf}}
	UMLXMI.png}}
	\caption{Input Class Diagram in XMI \label{fig:conceptual_m}}
\end{minipage}
\hfill
\begin{minipage}[b]{.320\linewidth}
    \fcolorbox{black}{white}{\includegraphics[width=1\linewidth]{BDA2020_Demo/images/%instance_5F.pdf}}
    CMMXMI.png}}
    \caption{5Families model in XMI \label{fig:logical_m}}
\end{minipage}
\hfill
\begin{minipage}[b]{.320\linewidth}
    \fcolorbox{black}{white}{\includegraphics[width=1\linewidth]{BDA2020_Demo/images/%instance_mongodb.pdf}}
    MongoDBXMI.png}}
    \caption{MongoDB model in XMI \label{fig:physical_m}}
\end{minipage}
\end{figure}
\end{comment}




==> BDA2020_Demo/files/06-Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Our \DG~approach is a MDA-based approach that aims to improve model transformation. \DG~is a global approach that generates optimized models based on the common \MMFF{} meta-model favoring the application of refinement rules to produce potential target models. This mix between data modeling and optimization rises to an approach that aims to find the efficient target model among the 5 families of data.

For future works, %we wish to create another refinement rule, whose goal is to transform a \texttt{Reference} into an \texttt{Edge} to incorporate \texttt{Graph Oriented} family.
we seek to define a generic cost model allowing to compare the produced solutions and eventually suggest top-k logical models. This cost model will integrate different dimensions (storage, bandwidth, CPU/energy impact, etc.) and will help to make a decision among all produced data models.  

==> EDBT/02-State_of_the_Art.tex <==
\section{Related Works}
\label{sec:related works}

%\remJ{talk about denormalization related works briefly}
In the literature, several works have discussed the costs of data models. 
Some of them have considered query execution time as its cost, some considered the financial cost, while others took into account the environmental impact of each query.

%\remJ{Target Data Model, Data Model Transformation}

\paragraph{Data Model Choice}

Many existing works have tackled the issue of transforming a current data model to a new one that is more appropriate to handle the fast-growing data.
They transform to data models conform to one or multiple NoSQL families.

Some of these approaches transform a relational data model into one data model of on target NoSQL family (to \texttt{CO}~\cite{vajk2013}, \texttt{DO}~\cite{rocha2015} or \texttt{GO}~\cite{daniel2016umltographdb}).

Moreover, other studies choose to transform into one or multiple physical solutions.
Chebotko et al.~\cite{chebotko2015} propose an approach to model \textit{Cassandra}.

Finally, other %dedicated 
approaches transform to one of the four NoSQL families, using either conceptual mapping~\cite{claudino2016} or Model-Driven Architecture (MDA)~\cite{abdelhedi2017}.

%\remNT{Orienter sur la question du choix du data model }
%\remNT{orienter sur "modèle de coût logique" indépendant des contraintes inhérentes à la solution logiciel (NoSQL)}

%\remJ{talk cost models in the literature, they focus on the query cost for query optimization}


\paragraph{Query's Cost Model}
%\remJ{Query's Cost Model}
%\remNT{Cost Model for Query Optimization}

In the literature, cost models have been used in the context of query optimization. The focus was always on query's cost where some works studied the time cost of a query while others focused on its environmental impact.

In terms of time cost, some papers have considered the time to execute a query to compare execution plans. 
In~\cite{ozsu1999}, the authors express the cost of a distributed execution strategy with respect to either the total time or the response time. The total time is the sum of all time (also referred to as cost) components, while the response time is the elapsed time from the initiation to the completion of the query. The cost includes the local processing time (time of a CPU instruction and the time of a disk I/O) and the communication time (the fixed time of initiating and receiving a message and the time it takes to transmit a data unit from one site to another).
In~\cite{sellami2017}, the authors define the cost of an execution plan as the sum of the cost of each operation (\textit{i.e.,} node in the execution plan) composing an execution plan. This cost depends at least on one of the three costs that are the CPU cost, the input/output cost, and the communication cost.

\paragraph{Environmental cost of IS}
Other papers focus on the impact of carbon footprint on the environment. Due to processing huge amounts of data, the energy consumed by the Cloud servers can lead to a huge amount of carbon emission with environmental impacts.
In~\cite{thakur2016carbon}, the authors discuss some technologies to reduce the energy consumption and carbon footprint of data centers. They also define metrics for measuring the carbon emission. 
In~\cite{rodriguez2011}, the authors develop a cost model to estimate the power and energy cost of database queries using multilinear regression. They don't make the power/energy measurements on individual hardware components (\textit{e.g.,} CPU, RAM, HD). Instead, the cost models are derived from: a) measurements taken from internal sensors, or a power meter attached to the server enclosure, and b) readily available workload statistics such as relation cardinality, tuple size, number of columns and number of servers.
In~\cite{saraiva2017}, the authors aim to evaluate the energy consumption of different types of queries, and at the same time compare it in terms of relational and non-relational database approaches (MySQL, Neo4j).
In~\cite{mahajan2019}, the authors study query optimization techniques that can improve energy efficiency without compromising performance of relational and NoSQL databases. 
%They use Speedup (the ratio of the execution time of the un-optimized query over the execution time of the optimized query), Powerup (the ratio of the average power consumed by the optimized query over the average power consumed by the un-optimized query) and Greenup (the ratio of the energy consumption of the un-optimized query over the energy consumption of the optimized query) metrics to compare query optimzations.

\bigskip

\modifNT{Conclusion sur : Critiquer les approches et dire qu'il manque un modele de cout pour orienter vers le choix du data model

As far as we know, no DataModel-based Cost Model... taking into account both data model (independent of queries) and query costs.

Goal: Having a comprehensive cost model, global view for a decision of the proper data model which minimize the query cost finally}

